HINT: A Hierarchical Index for Intervals in Main Memory

Indexing intervals is a fundamental problem, finding a wide range of applications. Recent work on managing large collections of intervals in main memory focused on overlap joins and temporal aggregation problems. In this paper, we propose novel and efficient in-memory indexing techniques for intervals, with a focus on interval range queries, which are a basic component of many search and analysis tasks. First, we propose an optimized version of a single-level (flat) domain-partitioning approach, which may have large space requirements due to excessive replication. Then, we propose a hierarchical partitioning approach, which assigns each interval to at most two partitions per level and has controlled space requirements. Novel elements of our techniques include the division of the intervals at each partition into groups based on whether they begin inside or before the partition boundaries, reducing the information stored at each partition to the absolutely necessary, and the effective handling of data sparsity and skew. Experimental results on real and synthetic interval sets of different characteristics show that our approaches are typically one order of magnitude faster than the state-of-the-art.

==> sections/flat.tex <==
\section{Flat Indexing}
\label{sec:flat}

%Notation: \\
%$P.st, P.end$: start-, end- endpoint of partition $P$.

In this section, we propose a single-level indexing approach (termed FLAT), based on disjoint partitions, which also serves as building block for our hierarchical index, presented in Section \ref{sec:hierarchical}. FLAT is inspired by partitioning approaches for interval joins (e.g., \cite{BourosM17,GunadhiS91}) and spatial joins (e.g., \cite{DittrichS00}).
Besides presenting a basic version of FLAT, stemming directly from previous work, we propose a number of optimizations, which greatly improve its efficiency in practice.
Table \ref{table:notations} summarizes the notations used throughout the paper.

\begin{table}[ht]
\caption{Table of notations\label{table:notations}}
\vspace{-0.2cm}
\centering
\footnotesize
%\begin{tabular}{|c|p{5.3cm}|}
\begin{tabular}{|c|c|}
\hline
\textbf{notation} &\textbf{description}\\ % 
\hline\hline
$s.id, s.st, s.end$ &identifier, start, end point of interval $s$ \\
$q=[q.st, q.end]$ &query range interval\\
$P_i$ & $i$-th domain partition and its contents\\
$P_i.st, P_i,end$ & start, end point of $i$-th domain partition\\
$P_i^O$ ($P_i^R$) & sub-partition of $P_i$ with originals (replicas)\\
\rule{0pt}{4ex}  $P_i^{O_{in}}$ ($P_i^{O_{aft}}$) & intervals in $P^O_i$ ending inside (after) partition $P_i$\\
%  $m$ & number of levels in 
  $P_{\ell,i}$ & $i$-th partition at level $\ell$ of HINT index\\
  $prefix(k, x)$ & $k$-bit prefix of integer $x$\\  
\hline
\end{tabular}
\end{table}

\subsection{Basic Version of FLAT}
\label{sec:flat:basic}
FLAT divides the domain into $p$ partitions
% \nikos{changed $m$ to $p$ because $m$ is used later to denote the number of levels at HIER},
$P_1,P_2,\dots,P_p$, which
are pairwise disjoint in terms of their interval span and collectively cover the entire data domain $D$; that is (i) for each $i,j: 1\le i<j\le p$, we have 
$[P_i.st,P_i.end] \cap [P_j.st,P_j.end] = \emptyset$, and (ii) $\bigcup_{i=1\dots p}[P_i.st,P_i.end] = D$.%
\footnote{Whenever the context is clear, we use the same symbol $P_i$ to denote the contents of partition $P_i$ and the interval that defines it. For example, we use $P.st, P.end$ to denote the start and end value of the domain interval corresponding to partition $P$.}
Domain partitioning could be regular (i.e., uniform) or may adapt to the data distribution (e.g., see \cite{BourosM17}).

Each interval $s\in S$ is assigned to all partitions that $s$ overlaps with. For example, assume that the domain $D$ is divided into $p=4$ partitions and consider a set $S$ with 5 intervals, as shown in Figure \ref{fig:flat}. Interval $s_1$ is assigned to partition $P_1$ only, whereas interval $s_5$ is assigned to all four partitions.
Given a range query interval $q$, the intervals that overlap with $q$ can be obtained by accessing the partitions which collectively cover $q$. For each partition $P_i$ which is contained in $q$ (i.e., $q.st\le P_i.st \wedge P_i.end\le q.end$), all intervals assigned to $P_i$ are guaranteed to overlap with $q$. For each partition $P_i$, which is not contained in $q$ but overlaps with $q$, we need to compare each interval $s_i \in P_i$ with $q$ in order to determine whether $s_i$ is a query result. Each partition that does not overlap with $q$ can be safely ignored. For example, for query interval $q$  in Figure \ref{fig:flat}, partitions $P_2$, $P_3$, and $P_4$ have to be accessed, wherefrom we obtain result $\{s_2,s_4,s_5\}$. Note that $s_3$, which is included in $P_2$ is not  a query result, as $s_3$ does not overlap with $q$.

One issue that arises in range query evaluation using FLAT is that duplicate results may be produced, which need to be handled. 
This may happen in the case where the query interval $q$ overlaps with multiple partitions.
%This case is expected to be frequent, because, for the partitioning approach to be effective, the number of partitions $p$ should be large and the extent of each partition small compared to a typical query.
For example, in Figure \ref{fig:flat}, $s_4$ can be identified as a result of query $q$ in all $P_2$, $P_3$, and $P_4$.
An efficient approach for handling duplicates (that does not rely on hashing) is the {\em reference value} method \cite{DittrichS00}, which was originally proposed for rectangles but can directly be applied for 1D intervals. For each interval $s$ found to overlap with $q$ in any partition $P_i$, we compute $v=\max\{s.st, q.st\}$ as reference value and report $s$ only if $v\in [P_i.st,P_i.end]$. Since $v$ is unique, $s$ is reported only in one partition and duplicate results are avoided. In Figure \ref{fig:flat}, $s_4$ is only reported in $P_2$ because $P_2$ contains value $\max\{s_4.st, q.st\}$.
Still, FLAT has the overhead that the duplicate results should be computed and considered before being eliminated by the reference value approach. In the next subsection, we show how the computation and elimination of duplicates can be completely avoided\eat{ overall}. In addition, we show how the necessary comparisons for each query can be minimized.

\begin{figure}[t]%[htb]
     \includegraphics[width=0.99\columnwidth]{figures/flat}
     \vspace{-2mm}
     \caption{Example of basic FLAT indexing}
  \label{fig:flat}
\end{figure}



\subsection{FLAT+}
\label{sec:flat:plus}
\eat{
  \panos{comments:
\begin{itemize}
\item We don't discuss at all the special case when $p_f = P_l$. We need to explicitly say then Lemma~1 and Lemma~2 don't hold in that case.
\item The basic version of FLAT+ can be further accelerated by sorting in combination with binary search; should we consider this? The reviewer may wonder why not. On the other hand, this is the case with all methods, even the linear scan.
\item The discussion for FLAT+ version with storage optimizations (let's call it FLAT+opts) is incomplete; you don't discuss how we store $P_i^{O_{aft}}$. The answer is of course similar to $P_i^{R_{aft}}$ as we only need the ids. But then, the FLAT+opts is not correct because in $P_l$ we need to perform comparisons for $P_l^{O_{aft}}$ and also, it doesn't cover the case when $P_f = P_l$.
\item To address this issue, currently in the implementation we also store $P_i^O$ and its triplets, which is used to check $P_l$; if $P_f = P_l$ then we perform two comparisons per interval while otherwise we compare only the start to q.end.
\end{itemize}
}
}
The key idea behind the FLAT+ index is to divide the intervals that are assigned to each partition into two groups, inspired by the re-partitioning approach proposed in \cite{BourosM17} for parallel processing of interval joins. 
In particular, for each partition $P$, all intervals that start inside but not before $P.st$, i.e., the starting endpoint of the \eat{$P$ }partition, are placed into set $P^O$ (for {\em originals}) while those which start before $P.st$ are placed into set $P^R$ (for {\em replicas}).
Figure \ref{fig:flatplus} shows the contents of $P_i^O$ and $P_i^R$, $i=\{1,2,3,4\}$, for each of the four partitions in  Figure \ref{fig:flat}.
%+ Show example. A set $S$ of intervals. Each interval $s\in S$ is assigned to the partitions it intersects. 

Given a range query interval $q$, for the first partition $P_{f}$ that overlaps with $q$, we consider all intervals in $P_{f}$ as possible query results, as usual. However, for all other partitions $P_{i}$ which overlap with $q$, where $i>f$, we only need to consider the intervals in $P_i^O$ and we can safely disregard the entire set $P_i^R$. This is because, each interval in $P_i^R$ is guaranteed to overlap with $q$ in the previous partition $P_{i-1}$, hence it would definitely be a duplicate result in $P_i$. Consider again query $q$ in Figure \ref{fig:flat}. In partition $P_f =P_2$, we should consider all intervals, i.e.,  both $P_2^O$ and $P_2^R$. On the other hand, in partitions $P_3$ and $P_4$, we only consider all intervals in  $P_3^O$ and $P_4^O$ and ignore 
$P_3^R$ and $P_4^R$, respectively.
Recall that for the first partition ($P_2$) and the last one ($P_4$) we have to perform comparisons between all intervals in them and $q$, in order to verify whether the intervals overlap with $q$, while for all partitions $P_i$ in-between (i.e., $P_3$) we just report all intervals in $P^O_i$ without any comparisons.
In Figure \ref{fig:flatplus}, the accessed divisions per partition for query $q$ 
are shown in bold. 

\begin{figure}[htb]
     \includegraphics[width=0.99\columnwidth]{figures/flatplus}
     \vspace{-2mm}
  \caption{FLAT+ partitioning}
  \label{fig:flatplus}
\end{figure}

%Besides diving the contents of each partition $P$ into $P^O$ and $P^R$ and applying the aforementioned search approach,
In the rest of this section, we propose a number of additional optimizations that further improve the performance of FLAT indexing;
% nterval range queries which access multiple partitions.
these optimizations target interval range queries and are not relevant to the problem of interval joins, so they were not considered in previous work \cite{BourosM17}.
%\panos{Not 100\% accurate, $P^{R_{aft}}$ was considered in \cite{BourosM17}.}

\eat{
\begin{figure}[htb]
  \begin{minipage}{.4\columnwidth}
    \centering
    \scriptsize
\vspace{0.1in}
$P_1^O = \{s_1,s_3,s_5\}, P_1^R= \emptyset$\\
$P_2^O= \{s_4\}, P_2^R =\{s_3,s_5\}$\\
$P_3^O=\{s_2\}, P_3^R = \{s_4,s_5\}$\\
$P_4^O= \emptyset, P_4^R = \{s_2,s_4,s_5\}$\\
\vspace{0.1in}
      \small{(a) originals and replicas}
    \end{minipage}
  \begin{minipage}{.55\columnwidth}
    \centering
    \scriptsize
$P_1^{O_{in}} = \{s_1\}, P_1^{O_{aft}}= \{s_3,s_5\}$\\
$P_2^{O_{aft}}= \{s_4\}, P_2^{R_{in}} =\{s_3\}, P_2^{R_{out}}\{s_5\}$\\
$P_3^{O_{aft}}=\{s_2\}, P_3^{R_{aft}} = \{s_4,s_5\}$\\
$P_4^{R_{in}} = \{s_2,s_4,s_5\}$\\
\vspace{0.05in}
      \small{(b) subdivisions}
  \end{minipage}
\vspace{-0.1in}
  \caption{FLAT+ partitioning}
  \label{fig:flatplus}
\end{figure}
}



\subsubsection{Subdivisions of $P_i^O$ and $P_i^R$}
\label{sec:flat:plus:subdivisions}
We further divide set $P_i^O$ into $P_i^{O_{in}}$ and $P_i^{O_{aft}}$, such that $P_i^{O_{in}}$ (resp. $P_i^{O_{aft}}$) includes the intervals from $P_i^O$ that {\em end} inside  (resp. {\em after})
partition $P_i$.
Similarly, $P_i^R$ is divided into $P_i^{R_{in}}$ and $P_i^{R_{aft}}$.

\stitle{Range queries that overlap with multiple partitions.}
Consider a range query $q$ which overlaps with a sequence of {\em more than one partitions}.
Let $P_f$ be the first partition overlapping with $q$ and  $P_l$, the last one ($P_f\ne P_l$). As already mentioned, we should consider all intervals in $P_f$ (i.e., both $P_i^O$ and $P_i^R$) for possible overlap with  $q$. However, since the query interval $q$ starts inside $P_f$ but  ends {\em after} $P_f$,
% all intervals $s\in P_f$ for which $s.end\ge q.st$ are query results. More
we have the following lemma:
\begin{lemma}\label{lem:pf}
% This means that:
%\begin{itemize}
%\item
  If $P_f\ne P_l$ (i) each interval $s$ in $P_f^{O_{in}} \cup P_f^{R_{in}}$ overlaps with $q$ iff $s.end\ge q.st$; and
%\item
 (ii)  all intervals $s$ in $P_f^{O_{aft}}$ and $P_f^{R_{aft}}$ are guaranteed to overlap with $q$.
  %and no comparisons for each such interval are needed.
%\end{itemize}
\end{lemma}
Hence, we need {\em just one comparison} for each interval in $P_f^{O_{in}} \cup P_f^{R_{in}}$, whereas we can report all intervals $P_f^{O_{aft}}\cup P_f^{R_{aft}}$ as query results {\em without any comparisons}.
For partitions between $P_f$ and  $P_l$, we just report intervals in $P_i^O$ (i.e., in $P_f^{O_{in}} \cup P_f^{O_{aft}}$) as results, without any comparisons. For the last partition $P_l$, we consider just  $P_l^O$, and perform {\em one comparison per interval}. Specifically:
\begin{lemma}\label{lem:pl}
%\begin{itemize}
%\item
  If $P_f\ne P_l$, each interval $s$ in $P_l^{O_{in}} \cup P_l^{O_{aft}}$
  overlap with $q$ iff $s.st\le q.end$. 
%\end{itemize}
\end{lemma}

\stitle{Range queries that overlap with a single partition.}
If $P_f = P_l$, i.e.,  the range query $q$ overlaps only one partition $P_f$, we can use following lemma in place of Lemmas~\ref{lem:pf} and \ref{lem:pl}:
\begin{lemma}\label{lem:1p}
If $P_f = P_l$ then
\begin{itemize}
\item each interval $s$ in $P_f^{O_{in}}$ overlaps with $q$ iff $s.st \le q.end \wedge q.st \leq s.end$,
\item each interval $s$ in $P_f^{O_{aft}}$ overlaps with $q$ iff $s.st \le q.end$,
\item each interval $s$ in $P_f^{R_{in}}$ overlaps with $q$ iff $s.end \ge q.st$,
\item all intervals in $P_f^{R_{aft}}$ overlap with $q$.
\end{itemize}
\end{lemma}

Overall, the subdivisions help us to minimize the number of intervals in $P_f$ and in $P_l$, for which we have to apply comparisons.
Figure \ref{fig:flatplusdecomp} shows the subdivisions which are accessed by query $q$
in each partition.
In partition $P_f=P_2$, all four subdivisions are accessed, but comparisons are needed only for intervals in $P_2^{O_{in}}$ and  $P_2^{R_{in}}$.
In partition $P_3$, all ``originals'' in  
$P_3^{O_{in}}$ and $P_3^{O_{aft}}$ are accessed and reported without any comparisons.
Finally, in $P_l=P_4$, all ``originals'' in  
$P_3^{O_{in}}$ and $P_3^{O_{aft}}$ are accessed and compared to $q$.

\begin{figure}[htb]
     \includegraphics[width=0.99\columnwidth]{figures/flatplusdecomp}
     \vspace{-2mm}
  \caption{Subdivisions in FLAT+}
  \label{fig:flatplusdecomp}
\end{figure}



\subsubsection{Sorting the intervals in each subdivision}
\label{sec:flat:plus:sorting}
% {\bf Sorting the intervals in each subdivision}
We can keep the intervals in each subdivision sorted,
in order to reduce the number of comparisons for queries that access them.
For example, let us examine the last partition $P_l$ that overlaps with a query $q$. If the intervals $s$ in $P_l^{O_{in}}$ are sorted based on their start endpoint (i.e., $s.st$), we can simply access and report the intervals until the first $s\in  P_l^{O_{in}}$, such that $s.st>q.end$. Or, we can perform binary search to find the first  $s\in  P_l^{O_{in}}$, such that $s.st> q.end$ and then scan and report all intervals before $s$.
Table \ref{tab:orderings} (second column) summarizes the sort orders for each of the four subdivisions of a partition that can be beneficial in range query evaluation. 
For  a subdivision $P_i^{O_{in}}$, intervals may have to be compared based on their start point (if  $P_i=P_f$), or based on their end point (if  $P_i=P_l$), or based on both points (if $P_i=P_f=P_l$). Hence, we choose to sort based on either $s.st$ or $s.end$ to accommodate two of these three cases.
For  a subdivision $P_i^{O_{aft}}$, intervals may only have to be compared based on their start point (if $P_i=P_l$).  
For  a subdivision $P_i^{R_{in}}$, intervals may only have to be compared based on their end point (if $P_i=P_f$).  
Finally, for  a subdivision $P_i^{R_{aft}}$, there is never any need
to compare the intervals,
%if such a subdivision is accessed (i.e., all intervals are reported as
%results without any comparisons); this means that
so, no order provides any search benefit.

\begin{table}
  \caption{Sort orders that can be beneficial}\label{tab:orderings}
\footnotesize
     \vspace{-2mm}
  \begin{tabular}{|l|l|l|}
    \hline
    {\bf subdivision} & {\bf beneficial sorting} & {\bf necessary data}\\
    \hline\hline
    $P_i^{O_{in}}$& by  $s.st$ or by  $s.end$ & $s.id, s.st, s.end$\\
\rule{0pt}{3ex}    $P_i^{O_{aft}}$& by  $s.st$ & $s.id, s.st$\\
 \rule{0pt}{3ex}   $P_i^{R_{in}}$& by  $s.end$ & $s.id, s.end$\\
 \rule{0pt}{4ex}   $P_i^{R_{aft}}$& no sorting & $s.id$\\ \hline  
  \end{tabular}
\end{table}



\subsubsection{Storage optimization}
\label{sec:flat:plus:decomposition}
%\todo{update storage and sorting for DSM, as per our last discussion}
So far, we have assumed that each interval $s$ is stored in the partitions whereto $s$ is assigned as a triplet $\langle s.id, s.st, s.end \rangle$.
However, if we split the partitions into subdivisions, as discussed in Section \ref{sec:flat:plus:subdivisions}, we do not need to keep all information
of the intervals in them. Specifically, as Lemmas \ref{lem:pf}, \ref{lem:pl}, and \ref{lem:1p} suggest, for each subdivision $P_i^{O_{in}}$, we may need to use
$s.st$ and/or $s.end$ for each interval $s\in P_i^{O_{in}}$, while for each subdivision $P_i^{O_{aft}}$, we may need to use $s.st$ for each $s\in P_i^{O_{in}}$, but we will never need $s.end$. From the intervals $s$ of each  subdivision $P_i^{R_{in}}$, we may need $s.end$, but we will never use $s.st$. Finally, for each  subdivision $P_i^{R_{in}}$, we just have to keep the $s.id$ identifiers of the intervals.
Table \ref{tab:orderings} (third column) summarizes the data that we need to keep from each interval in the subdivisions of each partition.
Since each interval $s$ is stored as ``original'' in just one
partition, but as replica in possibly multiple partitions, a lot of
space can be saved by storing only the necessary data, especially in
the case when the
%extents of the partitions are small and the
intervals span multiple partitions. 

\eat{
/*
As discussed in Section \ref{sec:flat:plus:sorting}, subdivisions $P_i^{O_{in}}$ can be sorted by $s.st$ to facilitate the case where $P_i=P_l$ or by $s.end$ to facilitate the case where $P_i=P_f$. One way to improve search efficiency, is to trade space in order to serve both cases. Specifically, we can sort original triplets $\langle s.id, s.st, s.end \rangle$ in $P_i^{O_{in}}$ by $s.st$ to facilitate cases $P_i=P_l$ and $P_i=P_l=P_f$ and create a {\em replica} of $P_i^{O_{in}}$, where we store for each $s\in P_i^{O_{in}}$ pairs $\langle s.id, s.end \rangle$ sorted by $s.end$. Hence, if $P_l\ne P_f$, i.e., the query spans multiple partitions, we use the replica of $P_f^{O_{in}}$ (sorted by $s.end$) and the original $P_l^{O_{in}}$ (sorted by $s.st$). */
\todo{KILL THIS}
}

\eat{
      We can reduce the storage requirements and accelerate query evaluation at the same time, by {\em decomposing} each triplet and storing only the necessary decompositions per subdivision. Specifically:
      
\begin{itemize}
\item For all intervals in a subdivision $P_i^{O_{in}}$, we keep a table of
  $\langle s.st, s.id\rangle$ tuples sorted by $s.st$. If  $P_i=P_l$ (i.e., $P_i$ is the last partition overlapping with the query $q$), then, based on Lemma \ref{lem:pl}, we can use the sorted table to minimize the number of comparisons required for finding the intervals in   $P_i^{O_{in}}$ that overlap with $q$ (i.e., by applying binary search, or by scanning the table until we find a $s.st>q.end$).
  For subdivision $P_i^{O_{in}}$, we also keep a table of  $\langle s.end, s.id\rangle$ tuples sorted by $s.end$. If  $P_i=P_f$ (i.e., $P_i$ is the first partition intersecting the query $q$), then, based on Lemma \ref{lem:pf}, we can use the sorted table to minimize the number of comparisons required for finding the intervals in $P_i^{O_{in}}$ that overlap with $q$. \panos{For $P_i^{O_{aft}}$?}
\item For all intervals in a subdivision $P_i^{R_{in}}$, we keep a table of  $\langle s.end, s.id\rangle$ tuples sorted by $s.end$. If  $P_i=P_f$ (i.e., $P_i$ is the first partition intersecting the query $q$), then, based on Lemma \ref{lem:pf}, we can use the sorted table to minimize the number of comparisons required for finding the intervals in $P_i^{O_{in}}$ that overlap with $q$.
\item All intervals in a subdivision $P_i^{R_{aft}}$ start before and end after $P_i$. The endpoints of these intervals are never used (for comparisons) in query evaluation. Hence, for each $P_i^{R_{aft}}$, we only keep a table with the $s.id$'s of the intervals $s\in P_i^{R_{aft}}$.
\end{itemize}
With the aforementioned storage scheme, we greatly reduce the storage requirements for the partitions $P_i^{R}$ storing the replicas of the intervals. Specifically, for each replica $s$, instead of holding the entire triplet $\langle s.id, s.st, s.end \rangle$, we either keep  $\langle s.end, s.id \rangle$ (if the replica is in $P_i^{R_{in}}$) or just keep $s.id$ (if the replica is in $P_i^{R_{aft}}$). For  partitions $P_i^{O}$ holding originals, we slightly increase the storage by splitting triplet $\langle s.id, s.st, s.end \rangle$ to $\langle s.st, s.id \rangle$ and $\langle s.end, s.id \rangle$, but this helps us to greatly improve query performance.

\todo{add a richer example where the benefits of subdivision and decomposition become obvious to the lazy reader}
}




%\subsection{Preliminary Evaluation}
\subsection{Evaluation of FLAT+}
\label{sec:flat:exps}
%\nikos{I'm thinking of an experimental evaluation here between the different versions of the FLAT, in order to convince the reader about the value of the re-partitioning and the decomposition. From thereon we can just use FLAT+ in the experiments where we compare with the hierarchical index. To be discussed...//}

We now evaluate the four FLAT+ versions and FLAT
(Section~\ref{sec:flat:basic}).
%;
%we implemented all indices in
%\texttt{C++} and compiled them using \texttt{gcc} (v4.8.5) with flags
%\texttt{-O3}, \texttt{-mavx} and \texttt{-march=native}.
In particular, we denote by (i) FLAT+(base),
the version described in the introductory text of
Section~\ref{sec:flat:plus} which stores the intervals of a partition
$P_i$ inside the $P^O_i$ and $P^R_i$ sets, (ii) FLAT+subs, the version
which employs the subdivisions $P^{O_{in}}_i$, $P^{O_{aft}}_i$,
$P^{R_{in}}_i$, $P^{R_{aft}}_i$ discussed in
Section~\ref{sec:flat:plus:subdivisions}, (iii) FLAT+subs+sort, the
version described in Section~\ref{sec:flat:plus:sorting} which sorts
the intervals inside the subdivisions, and (iv) FLAT+subs+sort+sopt,
the version discussed in Section~\ref{sec:flat:plus:decomposition} for
storage optimization. For the comparison, we used datasets BOOKS and
TAXIS which represent inputs with long and short
intervals, respectively, and run 10K randomly distributed queries
while varying the number of partitions and the extent of each query as
a percentage of the domain size.
For more details about the
implementation and compilation options, our machine, and the
datasets and queries,
%and experimentation
%our
%experimental datasets
please refer to Section~\ref{sec:exps} and
Table~\ref{tab:datasets}.
%The experiments were conducted on a machine with 384 GBs of RAM and a
%dual Intel(R) Xeon(R) CPU E5-2630 v4 clocked at 2.20GHz running
   %    CentOS Linux 8.2.2004.
Figure~\ref{fig:flat_exps} reports the results;
%\footnote{Due to lack of space, we omit the plots on indexing time; nevertheless, the results follow the same trend as the index size reports.};
for the plots in Figures~\ref{fig:flat_exps}(e) and \ref{fig:flat_exps}(f), the number of partitions are set equal to the best value observed in Figures~\ref{fig:flat_exps}(b) and \ref{fig:flat_exps}(c), respectively.

The plots clearly show the efficiency of FLAT+ indexing and the merit of the proposed optimizations; all FLAT+ versions steadily outperform FLAT. Overall, we observe that FLAT+subs+sort+sopt is the fastest FLAT+ version while always being an order of magnitude faster than basic FLAT. For datasets with long-lived intervals such as BOOKS, FLAT+subs+sort+sopt achieves an order of magnitude higher throughput than FLAT+(base) and up to 3 times  higher throughput compared to FLAT+subs and FLAT+subs+sort. On the other hand, for datasets with very short intervals like TAXIS, the advantage of FLAT+subs+sort+sopt is smaller especially compared to FLAT+subs+sort mainly due to the low replication ratio. Nevertheless, FLAT+subs+sort+sopt is still the fastest FLAT+ version. The benefits from the storage optimizations discussed in Section~\ref{sec:flat:plus:decomposition} are twofold. As expected, the index always occupies less space; Figures~\ref{fig:flat_exps}(a), \ref{fig:flat_exps}(b) clearly show this. In addition though, the query evaluation is accelerated because FLAT+subs+sort+sopt incurs a smaller footprint in main memory and so, a higher cache hit ratio. 

In view of the above, we consider only the FLAT+subs+sort+sopt version for the rest of the text, simply denoting it as FLAT+.



\eat{
\subsection{Discussion}
\label{sec:flat:discussion}
Shortcomings of FLAT+ include the high storage requirements (even after the optimizations) if we want to have many partitions.
% One possible remedy is that the $P_i^{R_{aft}}$ id-tables can be compressed (I guess).
(We can also discuss here a comparison-free version of FLAT+, for the case where the domain is small and discrete. This can be compared with our precise hierarchical index. The only problem is that this may reduce the contribution of the next section.)
\panos{we can refer to Figure~\ref{fig:flat_exps} to prove our point}
}

%\begin{itemize}
%\item Describe 2-level, a.k.a. domain-based partitioning
%\item Discuss it as an adaptation of the spatial 2-level paper or connect to the interval joins papers \cite{BourosM17, BourosMTT20}
%\item Highlight shortcomings
%\end{itemize}


\begin{figure}[t]
%\vspace*{-2ex}
\begin{tabular}{cc}
BOOKS &TAXIS\\
\hspace{-1ex}\includegraphics[width=0.47\columnwidth]{plots/flat_isize_AARHUS-BOOKS_2013_c0_1_n10000_vary-p.pdf}
&\includegraphics[width=0.47\columnwidth]{plots/flat_isize_NYC-TAXIS_2013_c0_1_n10000_vary-p.pdf}
\\
%\hspace{-1ex}\includegraphics[width=0.47\columnwidth]{plots/flat_itime_AARHUS-BOOKS_2013_c0_1_n10000_vary-p.pdf}
%&\includegraphics[width=0.47\columnwidth]{plots/flat_itime_NYC-TAXIS_2013_c0_1_n10000_vary-p.pdf}
%\\
\hspace{-1ex}\includegraphics[width=0.47\columnwidth]{plots/flat_throughput_AARHUS-BOOKS_2013_c0_1_n10000_vary-p.pdf}
&\includegraphics[width=0.47\columnwidth]{plots/flat_throughput_NYC-TAXIS_2013_c0_1_n10000_vary-p.pdf}
\end{tabular}
\begin{small}
%\fbox{\parbox{220pt}
\fbox{\parbox{160pt}
{
\begin{center}
{\footnotesize FLAT}
%\hspace{0.5ex}
\includegraphics[width=0.06\columnwidth]{figures/0_05.pdf}
\hspace{1ex}
{\footnotesize FLAT+(base)}
%\hspace{0.5ex}
\includegraphics[width=0.06\columnwidth]{figures/0_25.pdf}
\hspace{1ex}
{\footnotesize FLAT+subs}
%\hspace{0.5ex}
\includegraphics[width=0.06\columnwidth]{figures/0_45.pdf}
%\hspace{1ex}
\\
{\footnotesize FLAT+subs+sort}
%\hspace{0.5ex}
\includegraphics[width=0.06\columnwidth]{figures/0_65.pdf}
\hspace{0.5ex}
{\footnotesize FLAT+subs+sort+sopt}
%\hspace{0.5ex}
\includegraphics[width=0.06\columnwidth]{figures/1.pdf}
%\hspace{1ex}
\end{center}
}
}
\end{small}
\begin{tabular}{cc}
\hspace{-1ex}\includegraphics[width=0.47\columnwidth]{plots/flat_throughput_AARHUS-BOOKS_2013_c0_1_n10000_vary-c_boxes.pdf}
&\includegraphics[width=0.47\columnwidth]{plots/flat_throughput_NYC-TAXIS_2013_c0_1_n10000_vary-c_boxes.pdf}
\end{tabular}
\vspace{-4mm}
\caption{Comparing FLAT variants}
\label{fig:flat_exps}
\end{figure}
